Neural Markov Logic Networks

We introduce neural Markov logic networks (NMLNs), a statistical relational learning system that borrows ideas from Markov logic. Like Markov logic networks (MLNs), NMLNs are an exponential-family model for modelling distributions over possible worlds, but unlike MLNs, they do not rely on explicitly specified first-order logic rules. Instead, NMLNs learn an implicit representation of such rules as a neural network that acts as a potential function on fragments of the relational structure. Similarly to many neural symbolic methods, NMLNs can exploit embeddings of constants but, unlike them, NMLNs work well also in their absence. This is extremely important for predicting in settings other than the transductive one. We showcase the potential of NMLNs on knowledge-base completion, triple classification and on generation of molecular (graph) data.

==> [2020]@arxiv-v3 - NMLN/table_molecules.tex <==

%\begin{table*}
%\begin{tabularx}{\textwidth}{ccc}
\begin{longtable}{|c|c|c|}
\caption{Novel Molecules existing in ChemSpider}
\label{tab:molecules_novel} \\ 
\hline
\textbf{Smile code} & \textbf{Molecule} & \textbf{Name}\\ 
\hline
\endfirsthead
\multicolumn{3}{c}%
{\tablename\ \thetable\ -- \textit{Continued from previous page}} \\ 
\hline
\textbf{Smile code} & \textbf{Molecule} & \textbf{Name} \\
\hline
\endhead





\begin{tabular}{l}CC(C)CCC(N)=O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/1.png}\end{tabular}& \begin{tabular}{l} 4-Methylpentanamide\end{tabular} \\ \hline 
\begin{tabular}{l}O=C(O)C1=CCCN1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/2.png}\end{tabular}& \begin{tabular}{l}Multiple search results\end{tabular} \\ \hline 
\begin{tabular}{l}O=C1CCCCN1O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/3.png}\end{tabular}& \begin{tabular}{l} 1-Hydroxy-2-piperidinone\end{tabular} \\ \hline 
\begin{tabular}{l}CC(N)CCC(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/4.png}\end{tabular}& \begin{tabular}{l} 4-AMINOVALERIC ACID\end{tabular} \\ \hline 
\begin{tabular}{l}CCCC(N)C(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/5.png}\end{tabular}& \begin{tabular}{l} DL-Norvaline\end{tabular} \\ \hline 
\begin{tabular}{l}CC(O)C(O)C(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/6.png}\end{tabular}& \begin{tabular}{l} 4-DEOXYTETRONIC ACID\end{tabular} \\ \hline 
\begin{tabular}{l}NCCCCCCO\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/7.png}\end{tabular}& \begin{tabular}{l} MO8840000\end{tabular} \\ \hline 
\begin{tabular}{l}CC(N)C(O)C(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/8.png}\end{tabular}& \begin{tabular}{l} 3-amino-2-hydroxybutanoic acid\end{tabular} \\ \hline 
\begin{tabular}{l}CC(CCN)C(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/9.png}\end{tabular}& \begin{tabular}{l} 4-Amino-2-methylbutanoic acid\end{tabular} \\ \hline 
\begin{tabular}{l}CC(=O)C=CC(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/10.png}\end{tabular}& \begin{tabular}{l} 4-Oxo-2-pentenoic acid\end{tabular} \\ \hline 
\begin{tabular}{l}CCC(O)CC(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/11.png}\end{tabular}& \begin{tabular}{l} 3-Hydroxyvaleric acid\end{tabular} \\ \hline 
\begin{tabular}{l}CCCCNC(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/12.png}\end{tabular}& \begin{tabular}{l} Butylcarbamic acid\end{tabular} \\ \hline 
\begin{tabular}{l}CCCC(=N)C(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/13.png}\end{tabular}& \begin{tabular}{l}Multiple search results\end{tabular} \\ \hline 
\begin{tabular}{l}CCCCC(=O)CO\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/14.png}\end{tabular}& \begin{tabular}{l} 1-Hydroxy-2-hexanone\end{tabular} \\ \hline 
\begin{tabular}{l}OCCCNCCO\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/15.png}\end{tabular}& \begin{tabular}{l} 3-((2-Hydroxyethyl)amino)propanol\end{tabular} \\ \hline 
\begin{tabular}{l}NC(=O)CCC(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/16.png}\end{tabular}& \begin{tabular}{l} 4-Amino-4-oxobutanoic acid\end{tabular} \\ \hline 
\begin{tabular}{l}O=C(O)C1C=CCC1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/17.png}\end{tabular}& \begin{tabular}{l} 2-Cyclopentenecarboxylic acid\end{tabular} \\ \hline 
\begin{tabular}{l}ONC1CCCCC1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/18.png}\end{tabular}& \begin{tabular}{l} NC3410400\end{tabular} \\ \hline 
\begin{tabular}{l}CC(C)CCCCO\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/19.png}\end{tabular}& \begin{tabular}{l} 5-Methyl-1-hexanol\end{tabular} \\ \hline 
\begin{tabular}{l}CC(=O)CCC(N)=O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/20.png}\end{tabular}& \begin{tabular}{l} 4-Oxopentanamide\end{tabular} \\ \hline 
\begin{tabular}{l}NC1CCCC(=O)C1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/21.png}\end{tabular}& \begin{tabular}{l} 3-Aminocyclohexanone\end{tabular} \\ \hline 
\begin{tabular}{l}O=NC1CCCCC1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/22.png}\end{tabular}& \begin{tabular}{l} Nitrosocyclohexane\end{tabular} \\ \hline 
\begin{tabular}{l}CCCCP(=O)(O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/23.png}\end{tabular}& \begin{tabular}{l} Butylphosphonate\end{tabular} \\ \hline 
\begin{tabular}{l}CC(C)COC(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/24.png}\end{tabular}& \begin{tabular}{l} Isobutyl hydrogen carbonate\end{tabular} \\ \hline 
\begin{tabular}{l}CCCCCNC=O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/25.png}\end{tabular}& \begin{tabular}{l} MFCD07784338\end{tabular} \\ \hline 
\begin{tabular}{l}CC(C)(O)CC(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/26.png}\end{tabular}& \begin{tabular}{l} 3-OH-isovaleric acid\end{tabular} \\ \hline 
\begin{tabular}{l}O=C1CCCCC1O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/27.png}\end{tabular}& \begin{tabular}{l} Adipoin\end{tabular} \\ \hline 
\begin{tabular}{l}CNCCCCCO\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/28.png}\end{tabular}& \begin{tabular}{l} MFCD16696454\end{tabular} \\ \hline 
\begin{tabular}{l}CCCC(C)C(C)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/29.png}\end{tabular}& \begin{tabular}{l} MFCD00021889\end{tabular} \\ \hline 
\begin{tabular}{l}CC(C)CCC(N)=S\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/30.png}\end{tabular}& \begin{tabular}{l} 4-Methylpentanethioamide\end{tabular} \\ \hline 
\begin{tabular}{l}O=C(O)C1C=CC=N1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/31.png}\end{tabular}& \begin{tabular}{l}Multiple search results\end{tabular} \\ \hline 
\begin{tabular}{l}CCCCCC(C)C\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/32.png}\end{tabular}& \begin{tabular}{l} 2-Methylheptane\end{tabular} \\ \hline 
\begin{tabular}{l}CC(C)C=CC(N)=O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/33.png}\end{tabular}& \begin{tabular}{l} 4-Methyl-2-pentenamide\end{tabular} \\ \hline 
\begin{tabular}{l}COCCCC(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/34.png}\end{tabular}& \begin{tabular}{l} 4-Methoxybutanoic acid\end{tabular} \\ \hline 
\begin{tabular}{l}NCCC(=O)C(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/35.png}\end{tabular}& \begin{tabular}{l} 4-Amino-2-oxobutanoic acid\end{tabular} \\ \hline 
\begin{tabular}{l}NCC(=O)CC(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/36.png}\end{tabular}& \begin{tabular}{l} 4-Amino-3-oxobutanoic acid\end{tabular} \\ \hline 
\begin{tabular}{l}CCCC=CC(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/37.png}\end{tabular}& \begin{tabular}{l} 2-Hexenoic acid\end{tabular} \\ \hline 
\begin{tabular}{l}CCCCCC(O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/38.png}\end{tabular}& \begin{tabular}{l} Hexanediol\end{tabular} \\ \hline 
\begin{tabular}{l}CCCC(=O)C(C)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/39.png}\end{tabular}& \begin{tabular}{l} 2-Hydroxy-3-hexanone\end{tabular} \\ \hline 
\begin{tabular}{l}CC(CO)CC(N)=O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/40.png}\end{tabular}& \begin{tabular}{l} 4-Hydroxy-3-methylbutanamide\end{tabular} \\ \hline 
\begin{tabular}{l}CCCCCC(=N)N\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/41.png}\end{tabular}& \begin{tabular}{l} Hexanamidine\end{tabular} \\ \hline 
\begin{tabular}{l}CC1CCC1C(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/42.png}\end{tabular}& \begin{tabular}{l} 2-Methylcyclobutanecarboxylic acid\end{tabular} \\ \hline 
\begin{tabular}{l}NC(CCO)C(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/43.png}\end{tabular}& \begin{tabular}{l} Homoserine\end{tabular} \\ \hline 
\begin{tabular}{l}O=C1CC=CC=C1O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/44.png}\end{tabular}& \begin{tabular}{l}Multiple search results\end{tabular} \\ \hline 
\begin{tabular}{l}CC(C)CCCCN\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/45.png}\end{tabular}& \begin{tabular}{l} 5-Methyl-1-hexanamine\end{tabular} \\ \hline 
\begin{tabular}{l}NC1=CC=CC(=O)C1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/46.png}\end{tabular}& \begin{tabular}{l}Multiple search results\end{tabular} \\ \hline 
\begin{tabular}{l}CNC1CCCCC1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/47.png}\end{tabular}& \begin{tabular}{l} GX1529000\end{tabular} \\ \hline 
\begin{tabular}{l}CCCC1=CC(=O)C1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/48.png}\end{tabular}& \begin{tabular}{l} 3-Propyl-2-cyclobuten-1-one\end{tabular} \\ \hline 
\begin{tabular}{l}ClC1=CCCCCC1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/49.png}\end{tabular}& \begin{tabular}{l} 1-Chlorocycloheptene\end{tabular} \\ \hline 
\begin{tabular}{l}CCCCOC(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/50.png}\end{tabular}& \begin{tabular}{l} monobutyl carbonate\end{tabular} \\ \hline 
\begin{tabular}{l}O=C(Cl)CC1C=CC1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/51.png}\end{tabular}& \begin{tabular}{l} Cyclobutylideneacetyl chloride\end{tabular} \\ \hline 
\begin{tabular}{l}CC(=O)CCCCN\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/52.png}\end{tabular}& \begin{tabular}{l} 6-Amino-2-hexanone\end{tabular} \\ \hline 
\begin{tabular}{l}CCNC(C)C(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/53.png}\end{tabular}& \begin{tabular}{l} N-Ethylalanine\end{tabular} \\ \hline 
\begin{tabular}{l}N=C1CCCCN1O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/54.png}\end{tabular}& \begin{tabular}{l} 2-Imino-1-piperidinol\end{tabular} \\ \hline 
\begin{tabular}{l}CCCC=CC(N)=O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/55.png}\end{tabular}& \begin{tabular}{l} (2E)-2-Hexenamide\end{tabular} \\ \hline 
\begin{tabular}{l}NCCC1=CC(=O)C1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/56.png}\end{tabular}& \begin{tabular}{l}Multiple search results\end{tabular} \\ \hline 
\begin{tabular}{l}CCC(C)CC(N)=O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/57.png}\end{tabular}& \begin{tabular}{l} 3-Methylpentanamide\end{tabular} \\ \hline 
\begin{tabular}{l}NC(=O)C1CCCC1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/58.png}\end{tabular}& \begin{tabular}{l} Cyclopentanecarboxamide\end{tabular} \\ \hline 
\begin{tabular}{l}CCCCC(C)CC\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/59.png}\end{tabular}& \begin{tabular}{l} 3-Methylheptane\end{tabular} \\ \hline 
\begin{tabular}{l}CCCC(O)C(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/60.png}\end{tabular}& \begin{tabular}{l} 2-hydroxyvaleric acid\end{tabular} \\ \hline 
\begin{tabular}{l}O=C1C=CC(O)=CC1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/61.png}\end{tabular}& \begin{tabular}{l} 4-(2H)Hydroxy-2,4-cyclohexadien-1-one \end{tabular} \\ \hline 
\begin{tabular}{l}O=C(O)C1CC=CC1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/62.png}\end{tabular}& \begin{tabular}{l} 3-Cyclopentenecarboxylic Acid\end{tabular} \\ \hline 
\begin{tabular}{l}OCC1CCCCC1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/63.png}\end{tabular}& \begin{tabular}{l} Cyclohexylmethanol\end{tabular} \\ \hline 
\begin{tabular}{l}CC(CO)CCCN\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/64.png}\end{tabular}& \begin{tabular}{l} 5-Amino-2-methyl-1-pentanol\end{tabular} \\ \hline 
\begin{tabular}{l}CC1CCCC(N)N1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/65.png}\end{tabular}& \begin{tabular}{l} 6-Methyl-2-piperidinamine\end{tabular} \\ \hline 
\begin{tabular}{l}CCC(=O)CC(N)=O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/66.png}\end{tabular}& \begin{tabular}{l} 3-Oxopentanamide\end{tabular} \\ \hline 
\begin{tabular}{l}CC(O)CCCCN\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/67.png}\end{tabular}& \begin{tabular}{l} 6-Amino-2-hexanol\end{tabular} \\ \hline 
\begin{tabular}{l}NC1CC=CC(=O)C1\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/68.png}\end{tabular}& \begin{tabular}{l}Multiple search results\end{tabular} \\ \hline 
\begin{tabular}{l}CCNCCCCO\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/69.png}\end{tabular}& \begin{tabular}{l} 4-(Ethylamino)-1-butanol\end{tabular} \\ \hline 
\begin{tabular}{l}NCCCCC(N)=O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/70.png}\end{tabular}& \begin{tabular}{l} 5-Aminopentanamide\end{tabular} \\ \hline 
\begin{tabular}{l}CCCCCC(=O)Cl\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/71.png}\end{tabular}& \begin{tabular}{l} 506332\end{tabular} \\ \hline 
\begin{tabular}{l}CC(C)CNC(N)=O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/72.png}\end{tabular}& \begin{tabular}{l} Isobutylurea\end{tabular} \\ \hline 
\begin{tabular}{l}C=C(C)CCC(=O)O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/73.png}\end{tabular}& \begin{tabular}{l} 4-Methyl-4-pentenoic acid\end{tabular} \\ \hline 
\begin{tabular}{l}OC1=CCCCC1O\end{tabular} &  \begin{tabular}{l}\includegraphics[width=0.1\linewidth]{figs/table_figs/74.png}\end{tabular}& \begin{tabular}{l}Multiple search results\end{tabular} \\ \hline 
\end{longtable}
%\end{table*}
